TXS 0128+554: A Young Gamma-Ray Emitting AGN With Episodic Jet Activity

We have carried out a Chandra X-ray and multi-frequency radio VLBA study of the AGN TXS 0128+554, which is associated with the Fermi gamma-ray source 4FGL J0131.2+5547. The AGN is unresolved in a target 19.3 ks Chandra image, and its spectrum is well fit by a simple absorbed power law model, with no distinguishable spectral features. Its relatively soft X-ray spectrum compared to other CSOs may be indicative of a thermal emission component, for which we were able to obtain an upper temperature limit of kT = 0.08 keV. The compact radio morphology and measured advance speed of 0.32c +- 0.07c indicate a kinematic age of only 82 y +- 17 y, placing TXS 0128+554 among the youngest members of the compact symmetric object (CSO) class. The lack of compact, inverted spectrum hotspots and an emission gap between the bright inner jet and outer radio lobe structure indicate that the jets have undergone episodic activity, and were re-launched a decade ago. The predicted gamma-ray emission from the lobes, based on an inverse Compton-emitting cocoon model, is three orders of magnitude below the observed Fermi LAT flux. A comparison to other Fermi-detected and non-Fermi detected CSOs with redshift z<0.1 indicates that the gamma-ray emission likely originates in the inner jet/core region, and that nearby, recently launched AGN jets are primary candidates for detection by the Fermi LAT instrument.

==> tables/imagestats.tex <==
\begin{deluxetable*}{cccccccc} 
%\tablenum{1}
%\tablecolumns{8} 
%\tabletypesize{\scriptsize} 
\tablewidth{0pt}  
\tablecaption{\label{t:imagestats} VLBA Image Properties}
\tablehead{
\colhead{$\nu$} & \colhead{$I_\mathrm{tot}$}   &\colhead{$I_\mathrm{peak}$} &  \colhead{Maj.} &   \colhead{Min.} &   \colhead{PA}\ &  \colhead{$I_\mathrm{rms}$} & \colhead{$I_\mathrm{base}$} \\[-2ex] 
\colhead{(GHz)} & \colhead{(mJy)} & \colhead{(mJy$\ \mathrm{bm}^{-1}$)} & \colhead{(mas)} & \colhead{(mas)} & \colhead{($^\circ$)} & \colhead{(mJy$\ \mathrm{bm}^{-1}$)} & \colhead{(mJy$\ \mathrm{bm}^{-1}$)}
}
\decimalcolnumbers
\startdata 
2.3	&207	&79	&5.71	&4.42	&$-$10.2	&0.07	&0.30 \\
5	&162	&61	&2.21	&1.87	&0.3	&0.03	&0.10 \\
6.6	&151	&62	&1.63	&1.37	&$-$3.1	&0.04	&0.15 \\
8.4	&151	&64	&1.35	&1.12	&$-$9.0	&0.05	&0.16 \\
15.4	&114	&63	&0.70	&0.58	&$-$11.8	&0.04	&0.12 \\
22.2	&97	&84	&0.53	&0.45	&$-$8.8	&0.06	&0.20 \\
\enddata
\tablecomments{Columns are as follows: (1) observing frequency (GHz),
  (2) total cleaned flux density (mJy), (3) map peak (mJy per beam),
  (4) FWHM major axis of restoring beam (milliarcseconds), (5) FWHM
  minor axis of restoring beam (milliarcseconds), (6) position angle
  of major axis of restoring beam (degrees), (7) rms noise level of
  image (mJy per beam), (11) lowest I contour (mJy per beam).}
\end{deluxetable*}
